Simple-OPD: Demystifying Warm-up for On-policy Distillation

On-policy distillation (OPD) trains a student on its own rollouts with token-level supervision from teacher models, but its effectiveness can depend strongly on the warm-up stage before OPD. In this paper, we demystify warm-up for OPD from both data and training perspectives. For data, we find that effective warm-up relies on teacher-compatible chain-of-thought supervision, and that even incorrect teacher rollouts can provide comparable benefits to correct ones. This suggests that warm-up primarily transfers a teacher-compatible thinking pattern rather than merely correct answers. For training, we show that low-rank adaptation (LoRA) with a near-saturation training duration better balances in-domain adaptation and out-of-distribution generalization than full-parameter SFT. Based on these findings, we propose Simple-OPD, a plug-and-play initialization method that warms up the student on teacher-generated CoT with LoRA before OPD. Experiments across diverse settings demonstrate the effectiveness and robustness of Simple-OPD.

==> tables/case_study1.tex <==
\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{}p{0.98\linewidth}@{}}
\toprule
\textbf{Prompt.}\;
Let $x^{8}+3x^{4}-4=p_{1}(x)\,p_{2}(x)\dotsm p_{k}(x)$,
where each non-constant $p_{i}(x)$ is monic with integer coefficients
and cannot be factored further over the integers. Compute
$p_{1}(1)+p_{2}(1)+\dots+p_{k}(1)$.\quad
\textbf{Gold:} $10$.
\smallskip

\textit{Each row of the excerpts below is a step heading copied
verbatim from the response, with a one-line summary of what happens
in that step.
\tea{Blue} marks a step (or short cue) that teacher and warmup both
produce; \err{red} marks a step that is unique to no-warmup.}
\\
\midrule
\textbf{Teacher response.}\quad Predicts $\boxed{10}$\;\checkmark\\[2pt]
\emph{\tea{Alright, I have this problem to solve.
Let's break it down and understand what's being asked.}}\\[2pt]
\tea{\textbf{Step 1: Factor $x^{8}+3x^{4}-4$.}}
\emph{Substitute $y{=}x^{4}$; $y^{2}{+}3y{-}4{=}(y{+}4)(y{-}1)$;
factor $x^{4}{+}4{=}(x^{2}{+}2x{+}2)(x^{2}{-}2x{+}2)$
(\tea{``Let's verify''}: expand back \checkmark);
$x^{4}{-}1{=}(x{-}1)(x{+}1)(x^{2}{+}1)$; check discriminants of the
five factors, all irreducible. Factorisation is complete.}\\[2pt]
\tea{\textbf{Step 2: Evaluate Each Factor at $1$.}}
\emph{$0,\;2,\;2,\;5,\;1$.}\\[2pt]
\tea{\textbf{Step 3: Sum the Values.}}
\emph{$0+2+2+5+1=10$.}\\[2pt]
\tea{\emph{Wait, let's double-check.}\quad
\textbf{Verification of Factorization.}}
\emph{Re-derive each factor and re-sum; still $10$.
$\boxed{10}$.}
\\
\midrule
\textbf{Warmup response.}\quad Predicts $\boxed{10}$\;\checkmark\\[2pt]
\emph{\tea{Alright, I have this problem to solve.
Let's break it down and understand what's being asked.}}\\[2pt]
\tea{\textbf{Step 1: Factorize $x^{8}+3x^{4}-4$.}}
\emph{Substitute $y{=}x^{4}$; $y^{2}{+}3y{-}4{=}(y{+}4)(y{-}1)$;
so $x^{8}{+}3x^{4}{-}4{=}(x^{4}{+}4)(x^{4}{-}1)$;
$x^{4}{-}1{=}(x{-}1)(x{+}1)(x^{2}{+}1)$.}\\[2pt]
\tea{\textbf{Step 2: Factor $x^{4}+4$ over the integers.}}
\emph{Ansatz $(x^{2}{+}ax{+}b)(x^{2}{+}cx{+}d)$; solve
$a{=}\pm 2,\,b{=}d{=}2$; get $(x^{2}{+}2x{+}2)(x^{2}{-}2x{+}2)$
(\tea{``Let's verify''}: expand back \checkmark).}\\[2pt]
\tea{\textbf{Step 3: Verify irreducibility of each factor.}}
\emph{Each of the five factors has discriminant $-4<0$
(or is linear); all irreducible over $\mathbb{Z}$.}\\[2pt]
\tea{\textbf{Step 4: Compute $p_{1}(1)+\dots+p_{k}(1)$.}}
\emph{$5+1+0+2+2=10$.}\\[2pt]
\tea{\emph{Wait, let's double-check the calculations.}}\quad
\emph{Recompute each $p_{i}(1)$; still $10$.}\\[2pt]
\tea{\emph{Alternative Approach: verify by evaluating the entire
polynomial at $x=1$.}}
\emph{$1^{8}{+}3\cdot 1^{4}{-}4=0$, and the factor product
$5\times 1\times 0\times 2\times 2=0$ matches \checkmark.
$\boxed{10}$.}
\\
\midrule
\textbf{No-warmup response.}\quad Predicts $\err{\boxed{15}}$\;$\err{\times}$\\[2pt]
\emph{To solve the problem, we need to factor the polynomial
$x^{8}+3x^{4}-4$ into irreducible monic polynomials with integer
coefficients. Let's proceed step by step.}\\[2pt]
\err{\texttt{\#\#\#} \textbf{Step 1: Let $y=x^{4}$.}}
\emph{Polynomial becomes $y^{2}+3y-4$.}\\[2pt]
\err{\texttt{\#\#\#} \textbf{Step 2: Factor the quadratic in $y$.}}
\emph{$y^{2}+3y-4=(y+4)(y-1)$.}\\[2pt]
\err{\texttt{\#\#\#} \textbf{Step 3: Substitute back $y=x^{4}$.}}
\emph{$x^{8}+3x^{4}-4=(x^{4}+4)(x^{4}-1)$.}\\[2pt]
\err{\texttt{\#\#\#} \textbf{Step 4: Factor $x^{4}-1$.}}
\emph{$=(x-1)(x+1)(x^{2}+1)$.}\\[2pt]
\err{\texttt{\#\#\#} \textbf{Step 5: Factor $x^{4}+4$.}}
\emph{Sophie Germain identity gives
$(x^{2}+2x+2)(x^{2}-2x+2)$.}\\[2pt]
\err{\texttt{\#\#\#} \textbf{Step 6: Combine all factors.}}
\emph{Write
$(x^{4}{+}4)(x^{2}{+}2x{+}2)(x^{2}{-}2x{+}2)(x^{2}{+}1)(x{-}1)(x{+}1)$.
List irreducibility: item~5 states \emph{``\err{$x^{4}+4$: We
already factored it as $(x^{2}+2x+2)(x^{2}-2x+2)$}''}, yet the
list of ``irreducible factors'' still contains
$\err{(x^{4}+4)}$---\err{a total of $6$ factors} instead of $5$.}\\[2pt]
\err{\texttt{\#\#\#} \textbf{Step 7: Compute
$p_{1}(1)+\dots+p_{k}(1)$.}}
\emph{$2+0+2+5+1+\err{5}=\err{\boxed{15}}$.}\\[2pt]
\textcolor{purple}{[No ``Verify irreducibility'' step, no
``Wait, let's double-check'' pass, and no $P(1){=}0$ /
factor-product cross-check---all of which teacher and warmup
perform---so the double-counted $(x^{4}+4)$ (worth $+5$) survives
into the final sum.]}
\\
\bottomrule
\end{tabular}
\caption{Step-by-step skeletons of the three responses on MATH500
\texttt{intermediate\_algebra/279} (Level~5). Teacher and warmup
share the same \tea{blue} workflow---factor, (in warmup: an extra
``Factor $x^{4}{+}4$'' step, matching teacher's inline sub-derivation),
\emph{explicitly verify irreducibility}, evaluate, sum, and then a
\emph{``Wait, let's double-check''} pass---and both output $10$.
No-warmup flattens the workflow into $7$ \err{red} enumeration
steps with no verification or double-check pass, so its own list
that flags $x^{4}{+}4$ as ``already factored'' still ends up
counting it a $6$th time, inflating the sum to $15$. All step
headings and quotations are verbatim.}
\label{tab:case_pattern}
\end{table*}


